RescueAR: Augmented Reality Supported Collaboration for UAV Driven Emergency Response Systems

Emergency response events are fast-paced, noisy, and they require teamwork to accomplish the mission. Furthermore, the increasing deployment of Unmanned Aerial Vehicles (UAVs) alongside emergency responders, demands a new form of partnership between humans and UAVs. Traditional radio-based information exchange between humans during an emergency response suffers from a lack of visualization and often results in miscommunication. This paper presents a novel collaboration platform: RescueAR, which utilizes the paradigm of Location-based Augmented Reality to geotag, share, and visualize information. RescueAR aims to support the two-way communication between humans and UAVs, facilitate collaboration across diverse responders, and visualize scene information relevant to the rescue team's role. According to our feasibility study, a user study, followed by a focus group session with police officers, RescueAR can support rescue teams in developing the spatial cognition of the scene, facilitate the exchange of geolocation information, and complement existing communication tools during the UAV-supported emergency response.

==> sections/framework.tex <==




   








